Neural Point Process for Learning Spatiotemporal Event Dynamics

Learning the dynamics of spatiotemporal events is a fundamental problem. Neural point processes enhance the expressivity of point process models with deep neural networks. However, most existing methods only consider temporal dynamics without spatial modeling. We propose Deep Spatiotemporal Point Process (\ours{}), a deep dynamics model that integrates spatiotemporal point processes. Our method is flexible, efficient, and can accurately forecast irregularly sampled events over space and time. The key construction of our approach is the nonparametric space-time intensity function, governed by a latent process. The intensity function enjoys closed form integration for the density. The latent process captures the uncertainty of the event sequence. We use amortized variational inference to infer the latent process with deep networks. Using synthetic datasets, we validate our model can accurately learn the true intensity function. On real-world benchmark datasets, our model demonstrates superior performance over state-of-the-art baselines. Our code and data can be found at the https://github.com/Rose-STL-Lab/DeepSTPP.

==> secs/back.tex <==
\begin{figure*}[t!]
     \centering
     %\vspace{-10mm}
     \includegraphics[width=\linewidth]{figs/fig1.png}
     \vspace{-5mm}
     \caption{%\ry{replace with spatiotemporal points, shorten sequence length} 
     Visualization of  the intensity functions $\lambda^*(s,t)$ over space and time for spatiotemporal Hawkes process (top) and the spatiotemporal self-correcting process (bottom). The crosses mark the arrived events, and their sizes decrease as time goes.}
    \label{fig:example of stpp}
\end{figure*}

\vspace{-2mm}
\paragraph{Temporal Point Processes}
\label{sec:MTPP-limitation}
A temporal point process~(TPP)  models the number of events $N(a,b)$  that occurred during the half-open interval $(a, b]$, with $a < b$. It is characterized by a non-negative  intensity function given the history $\mathcal H_t := \{t_1, ..., t_n\}_{t_n \leq t}$ as:
\begin{equation}
\lambda^*(t):=  \lim_{\Delta t \to 0}\frac{\mathbb{E}[ N(t, t+\Delta t)|\mathcal H_{t}]}{ \Delta t}, .
\label{eqn:def_tpp}
\end{equation}
In other words, the probability of finding an event in an infinitesimal  time interval $(t, t+\Delta t]$.  Here we use the notation $*$ from \cite{daley2007introduction} to indicate that this density is conditional on the
past right up to but not including the present. An example of TPP is temporal Hawkes process, with the conditional intensity function:
$\lambda^*(t) = \mu + \sum_{i:t_i < t} g_1(t - t_i) : \mu > 0 $


% A marked temporal point process~(MTPP) models the intensity to also depend on the past events' information other than timing. It describes an event as a two-tuple $\{t, y\}$, where $t\in \R^+$ is the event timing and $y$ is the event's continuous or discrete feature, namely, the event marker. The history condition is then denoted as $\mathcal H_t = \{(t_1, y_1), (t_2,y_2), ... ,(t_n, y_n):t_n < t\}$.



% and $*$ is a shortcut for $\mathcal H_t$. $\lambda^*(t)$ is such defined that the probability of finding an event in the time interval $[t, t+\delta t)$ of infinitesimal width $\delta t$ is $\lambda^*(t) \delta t$. 
% As a result, $\lambda^*(t)$ can be intuitively seen as the average event rate.

% Let $f^*(t) := f(t | \mathcal H_t)$ denotes the conditional density of the next event timing since the last event $t_n$, and $F^*(t) := F(t| \mathcal H_t) = \int_{t_n}^t f^*(\tau) d\tau$ denotes the cumulative probability that the next event will arrive before time $t$. The relation $f^*(t) = \dfrac{\lambda^*(t)\delta t}{1-F^*(t)}$ yields $f^*(t) = \lambda^*(t) \exp \Big( -\int_{t_{n}}^t \lambda^*(\tau) d\tau \Big)$. 



\iffalse
\paragraph{Poisson Process} The Poisson process is the most basic temporal point process, with its intensity $\lambda(t)=\lambda \geq 0$ defined as a constant. 

% A nonhomogenous Poisson process is defined by a time-varying but not history-dependent intensity. Both are memoryless, since the $\mathcal H_s: s<t$ has no influence on $N(t) - N(s)$.

\paragraph{Hawkes Process}
The Hawkes process is characterized by the intensity $\lambda^*(t) = \mu +  \sum_{i:t_i < t} g_1(t - t_i) : \mu > 0$, where $g_1$ is the triggering kernel and is often implemented as the exponential decay function, $g_1(\Delta t) := \alpha \exp(-\beta \Delta t) : \alpha, \beta > 0$. The Hawkes process captures self-excitation, assuming the each past event has an additive, positive, and decaying influence over the intensity. 

\paragraph{Self-Correcting Process}
The Self-Correcting process is characterized by the intensity $\lambda^*(t) = \exp(\mu t- \sum_{t_i < t} \alpha) : \alpha, \mu > 0$. The Self-Correcting process captures self-inhibition, assuming the background intensity ($\mu t$) increases over time and the arrival of each new event decreases the intensity by a factor of $\exp(\alpha)$.

\paragraph{Renewal Process}
The Renewal process is a family of the temporal point process whose conditional intensity function only depends on the time since the most recent event, i.e., $\lambda^*(t) = g(t - t_N)$. The Renewal process captures self-reset; the arrival of a new event resets the intensity to $g(0)$.

\paragraph{Marked Temporal Point Process}
A marked temporal point process models the intensity to depend on the past events' features other than timing. It describes an event as a two-tuple $\{t, y\}$, where $t\in \R^+$ is the event timing and $y \in \mathcal Y$ is the event's other features, namely, the event marker. The history condition is then denoted as $\mathcal H_t = \{(t_1, y_1), (t_2,y_2), ... ,(t_N, y_N):t_N < t\}$.

\paragraph{Neural Temporal Point Process}
Multiple models have been proposed to incorporate the recurrent neural network into the Marked Temporal Point Process. Such models sequentially map the input event sequence $\{(t_i, y_i)\}$ to a sequence of hidden vectors $\{\mathbf h_i\}$ by learning a recurrent neural network. The hidden vectors are then used as parameters to model the conditional intensity function. Compared to the classic TPP models, the Neural-TPP imposes fewer prior assumptions over the sign and the analytic form of the intensity change caused by each event and, therefore, often achieves better performance over real-world datasets.
\fi







% \subsection{Limitation of Marked Temporal Point Process in Spatial Inference} \label{sec:MTPP-limitation}

% While an MTPP utilizes the past event markers, its intensity is uni-variate and can not be used for predicting the next event marker. Most Neural-MTPP models, e.g. \citet{Neural-Hawkes, zuo2020transformer} only consider marker inference when the markers are discrete. Discrete markers allow one to translate MTPP as a multivariate TPP, and predict as a classification problem. 


% appoach is to  treat space  as continuous ``markers'' and model  the \textit{ground process}  . That means, the space-time intensity function  can be factorized. $\lambda(s,t)=\lambda(t)f(s|t)$ with $f(s|t)$ being the probabilistic density function. 

% \zz{The resulting  loss function has two terms:  a negative log-likelihood (NLL) part for the time-intensity,  and a regression loss part for the  location. However, 
% Consider an earthquake model, in which each event results in an increase in intensity that depends on both the epicenter location and event time. Temporal point process would not be able capture such dynamics. }

% \adam{I do not the see the necessity for this paragraph. We can just say: The marker-based space prediction is severely limited by the discrete nature of marker. We can only forecast finite number of locations, while in real-life application the location prediction is conducted on continous space.}

% Consider an earthquake model, in which each event results in an increase of $\lambda^*(t)$ proportional to the earthquake magnitude. Regardless of the epicenter's location, the earthquake's contribution to the earthquake intensity would be roughly the same. \zz{A Neural-MTPP will treat the input past locations as zero-importance features when reducing the NLL. This is because the past locations are not part of the intensity function, it is sufficient to memorize the past earthquakes' magnitudes and timings. The past locations are encoded in the hidden vectors only when the model is reducing the MSE.} In such a case, a Neural-MTPP would not have any clear advantage over having a separate RNN for the next event location prediction.
% Due to existence of both time interval and spatial domain,  we define the counting process on the Cartesian product of both sets $N(\Delta \V{s}\times \Delta t)$.
\vspace{-2mm}

%  $B(\mathbf s, \delta \mathbf s)$ is $\lambda^*(\mathbf s, t) |B(\mathbf s + \delta \mathbf s)|\delta t$, where $|B(\mathbf s + \delta \mathbf s)|$ is the Lebesgue measure of the ball. 

% \paragraph{Relationship to TPP} When the locations of the events are disregarded, a STPP characterized by $\lambda^*(\mathbf s,t)$ is equivalent to a TPP characterized by $\lambda^*(t) = \int_{\mathcal S} \lambda^*(\mathbf s,t) d\mathbf s$. The conditional density of the new event location is denoted as $f^*(\mathbf s | t) := f^*(\mathbf s |t, \mathcal H_t)$, depending on the new event timing and the past events. As a result, $\lambda^*(\mathbf s, t)$ can be alternatively defined as $\lambda^*(\mathbf s, t) = f^*(\mathbf s| t) \lambda^*(t)$ \cite{daley2007introduction}.

% \paragraph{Learning and Inference} Given a STPP, the likelihood of observing a sequence $\{\mathbf s_i, t_i\}$ is $\prod_{i} f^*(\mathbf s_i, t_i)$. The expectations of next event's location and time are $\int_{t_n}^{\infty} \int_{\mathcal S}\mathbf s f^*(\mathbf s, t) d\mathbf s dt$ and $\int_{t_n}^{\infty} \int_{\mathcal S} t f^*(\mathbf s, t) d\mathbf s dt$, respectively. $f^*(\mathbf s, t)$ evaluates to
% \begin{equation}
%     f^*(\mathbf s, t) = f^*(\mathbf s | t) f^*(t) =  f^*(\mathbf s | t) \lambda^*(t)\exp \Big( -\int_{t_{n}}^t \lambda^*(\tau) d\tau \Big) = \lambda^*(\mathbf s, t) \exp \Big( -\int_{t_{n}}^t \lambda^*(\tau) d\tau \Big)
% \end{equation}
% It is worth-noting that if the formulation of $\lambda^*(\mathbf s, t)$ does not give $\lambda^*(t) = \int_\mathcal S \lambda^*(\mathbf s, t) d\mathbf s$ a closed form, the calculation of likelihood and expectation may incur triple numerical integration, which greatly increases the time complexity for learning and inference. 




\ryu{Figure 2 not referenced and explained }
% \subsubsection{Two Example Spatiotemporal Point Processes}
% \label{sec:STPP-examples}

% To demonstrate an STPP's flexibility in modeling spatiotemporal events' hidden dynamics, below, we present two representative examples of STPP with distinct behaviors.


% Note that the STSCP without spatial markers is not equivalent to a markless self-correcting process. (see Appendix \ref{app:tpp-examples})
%This is because the event influence over the intensity is multiplicative instead of additive.


% The STSCP can express such sequence by having a bimodal $g_0$ that peaks at the home and the work locations. An event at home increases the likelihood of the next event being at the workplace, and vice versa.



